Distributed Weighted Matching via Randomized Composable Coresets

Maximum weight matching is one of the most fundamental combinatorial optimization problems with a wide range of applications in data mining and bioinformatics. Developing distributed weighted matching algorithms is challenging due to the sequential nature of efficient algorithms for this problem. In this paper, we develop a simple distributed algorithm for the problem on general graphs with approximation guarantee of $2+\varepsilon$ that (nearly) matches that of the sequential greedy algorithm. A key advantage of this algorithm is that it can be easily implemented in only two rounds of computation in modern parallel computation frameworks such as MapReduce. We also demonstrate the efficiency of our algorithm in practice on various graphs (some with half a trillion edges) by achieving objective values always close to what is achievable in the centralized setting.

==> exp.tex <==



\section{Empirical Study}\label{sec:exp}



In this section, we report the results of evaluating our algorithm on
a number of publicly available datasets.  These datasets have varying sizes, ranging from about six million to half a trillion edges.
See Table~\ref{tab:dataset-size} in Appendix~\ref{app:exp} for more details on our datasets. 

\ssection{Datasets.} Three of our datasets (namely Friendster, Orkut, and LiveJournal, all taken from SNAP) are the {\em public} datasets used in evaluating a
hierarchical clustering algorithm in~\cite{BBDHKLM17} (they also have a fourth {\em private} dataset). Maximum weight matching is important in the context of hierarchical
clustering, because it can be used to generate a more balanced
hierarchy:  Iteratively find a maximum weight matching and contract
the edges of the matching.  Then the size of clusters at each level $k$ will be
nearly the same and equal to $2^k$. We also add
a fourth dataset of our own based on \emph{public} DBLP co-authorship~\cite{DBLP:MIT}: vertices
denote authors and edge weights denote the number of papers two researchers co-authored. Appendix~\ref{app:exp} contains 
more details on our datasets. 

\ssection{Implementation Details.} %Scalability: We run on big data.
We implement our algorithm on a real proprietary MapReduce-like cluster, i.e., no simulations, with tens to hundreds of machines,
depending on the size of the dataset. In our set-up, as in any standard MapReduce system, data is
initially stored in distributed storage (each edge on an arbitrary machine), and is then fed into the system and the output matching will be stored in a single file on one machine. To be more precise, our implementation follows
the approach in Theorem~\ref{THM:GREEDY}: we first compute a coreset on each machine using $\GreedyCoreset$ and then after combining the edges, we simply run the greedy algorithm
again to compute the final solution. As such, our algorithm can be seen as the distributed version of the 
{\em sequential} greedy algorithm for the weighted matching problem. Our
experiments verify that our coreset approach provides significant speed-ups with little quality loss compared to the sequential greedy algorithm, which complements our theoretical results in Theorems~\ref{thm:main} and~\ref{THM:GREEDY}.

The two main measures we are interested in are the \emph{quality} of the returned solution and the \emph{speed-up} of the algorithms compared to the sequential greedy algorithm: 

\begin{itemize}
	\item \emph{Quality.} Our coreset-based approach typically secures close to 99.5\% of the weight of the solution found by the sequential greedy algorithm (and slightly above this for the cardinality instead of weight). 
Table~\ref{tab:speedup} shows the quality of the solution obtained on each dataset separately. We emphasize that even though our theoretical proof in Theorem~\ref{THM:GREEDY} guarantees
 a 66\% performance (for the
coreset-based algorithm with greedy as post-processing compared to the sequential greedy
algorithm), we never lose more than 1--2\% in terms of the solution quality (see also Remark~\ref{rem:too-good} for a theoretical explanation of this phenomenon).


	\item \emph{Speed-up.} The speed-up achieved by our coreset-based approach varies significantly between the datasets---ranging from $3$x to $130$x---compared to the sequential greedy algorithm. The speed-up is larger for bigger graphs, where the coreset
	computation can really take advantage of the parallelism. Table~\ref{tab:speedup} provides the speed-up obtained on each dataset separately. 
\end{itemize}
 
 \begin{table}[h!]
\caption{Speed-up and relative solution quality of our coreset-based
  algorithm compared to the sequential greedy algorithm.\label{tab:speedup}}
\vspace{1mm}
\centering
\begin{tabular}{lccc}
\hline
{\bf Dataset} & {\bf Speed-up} & {\bf Weight} &
                                                                   {\bf Cardinality} \\
\hline
{Friendster} & 130x & 99.83\% & 99.74\% \\
{Orkut} & \phantom{0}17x & 98.90\% & 99.42\% \\
{LiveJournal} & \phantom{00}6x & 99.86\% & 99.79\% \\
{DBLP} & \phantom{00}3x & 99.55\% & 99.27\% \\
\hline
\end{tabular}
\end{table}

Appendix~\ref{app:exp} contains further details about different aspects of our experiments and Appendix~\ref{app:comp} gives empirical and theoretical comparison of our algorithm with prior ones. 
 

